Aggregated Learning: A Deep Learning Framework Based on Information-Bottleneck Vector Quantization

Based on the notion of information bottleneck (IB), we formulate a quantization problem called "IB quantization". We show that IB quantization is equivalent to learning based on the IB principle. Under this equivalence, the standard neural network models can be viewed as scalar (single sample) IB quantizers. It is known, from conventional rate-distortion theory, that scalar quantizers are inferior to vector (multi-sample) quantizers. Such a deficiency then inspires us to develop a novel learning framework, AgrLearn, that corresponds to vector IB quantizers for learning with neural networks. Unlike standard networks, AgrLearn simultaneously optimizes against multiple data samples. We experimentally verify that AgrLearn can result in significant improvements when applied to several current deep learning architectures for image recognition and text classification. We also empirically show that AgrLearn can reduce up to 80% of the training samples needed for ResNet training.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> tikz_equivalenceDiagram.tex <==
\usetikzlibrary{calc}
\begin{tikzpicture}[
>=latex,
node distance=5mm,
hv path/.style={to path={-| (\tikztotarget)}},
vh path/.style={to path={|- (\tikztotarget)}},
skip loop/.style={to path={-- ++(0,#1) -| (\tikztotarget)}},
vskip loop/.style={to path={-- ++(#1,0) |- (\tikztotarget)}},
startend/.style={
draw,
rectangle,
rounded corners=2mm,
minimum size = 6mm,
thick
},
ioput/.style = {
draw,
trapezium,
trapezium left angle=60, trapezium right angle=120,
inner sep = 5pt
},
 chuli/.style={
rectangle, draw=black, thick, fill=white,
      text width=6em, text ragged, minimum height=4em, inner sep=6pt
},
 panduan/.style={
 draw,
diamond,
minimum size=6mm,
shape aspect=3,
inner sep = 0.1pt,
thick,
font=\itshape
}
]

\node (a) [chuli] {IB \\ Quantization};
\node (a12) [chuli,right = 3 cm of a] {Solving \\ $R_{\rm IB-RD}(D)$};
\node (a13) [chuli,right = 3 cm of a12] {Solving \\ $R_{\rm IB-Learn}(A)$};
\node (a14) [chuli,right = 3 cm of a13] {IB \\ Learning};
\node (b21) [below = 1cm of a]{Implementation};
\node (b22) [chuli,below = 1cm of a12]{Scalar\\ IB\\ Quantizer};
\node (b23) [chuli,below = 1.12cm of a13]{Standard  \\ Neural Net};
\node (b24) [below = 1cm of a14]{Learning Framework};
\node (c32) [chuli,below = 0.875cm of b22]{Vector\\ IB\\ Quantizer};
\node (c33) [chuli,below = 1.12cm of b23]{Agr Learn\\(This paper)};
\node(c31)[below=1.5cm of b21]{};
\node (c34)[below=1.5cm of b24]{};
\node ()[ above right =-0.8cm and 0.5cm of a]{Optimization};
\node ()[ above right =-1.2cm and 0.5cm of a]{Problem};
\node ()[ above right =-0.8cm and 0.5cm of a12]{Equivalent};
\node ()[ above right =-1.2cm and 0.5cm of a12]{Theorem2};
\node ()[ above right =-0.8cm and 0.5cm of a13]{Optimization};
\node ()[ above right =-1.2cm and 0.5cm of a13]{Problem};
\node ()[ above right =-0.9cm and 0.5cm of b22]{Equivalent};
\node ()[ above right =-0.9cm and 0.5cm of c32]{Equivalent};

\path     (a) edge[->,thick]        (a12);
\path     (a) edge[->,thick]        (a12);z
\path           (a12) edge[<->,thick]      (a13)
        (a14) edge[->,thick]        (a13)
        (a14) edge[->,thick]        (b24)
        (b22) edge[<->,thick]        (b23)
        (c32) edge[->,thick]        (c33)
        (a) edge[->,thick]        (b21)
 (b21) edge[->,thick]        (c31)
 (b24) edge[->,thick]        (c34);
%\draw[->, >=latex', shorten >=2pt, shorten <=2pt, bend right=45] 
%(c31.east) -- ++(2,0) -- ++(0,1.86) --  (b22.west);
\draw[->,thick] 
(b21.south) |- ++(0,-1.5) -- ++(2,0)-- ++(0,1.245) --  (b22.west);
\draw[->,thick] 
(b21.south) |- ++(0,-1.5) -- ++(2,0)-- ++(0,-1.359) --  (c32.west);


\draw[->, thick] 
(b24.south) |- ++(0,-1.5) -- ++(-2,0)-- ++(0,1.24) --  (b23.east);
\draw[->, thick] 
(b24.south) |- ++(0,-1.5) -- ++(-2,0)-- ++(0,-1.37) --  (c33.east);


\end{tikzpicture}
